A Comparison of High-Dimensional Variable Selection Procedures for Electricity Spot Price Forecasting

The paper considers the problem of variable selection for forecasting electricity spot prices. High-dimensional methods such as LASSO and Elastic Net are widely used for this purpose, and while they exhibit strong predictive performance, their tendency to select over-parameterized models raises questions about interpretability. We evaluate the performance of six variable selection procedures, includingthe recently proposed Boosting Multiple Testing (BMT) method, using an extensive dataset from six regional electricity markets. We assess their performance in terms of both out-of-sample forecasting ac-curacy and model parsimony. We find that, although LASSO and Elastic Net achieve similar accuracy and outperform most screening alternatives, BMT matches their forecasting performance while using less than one-tenth as many variables. Our results reveal that BMT offers researchers and practitioners a substantially more interpretable and computationally efficient alternative to shrinkage methods, without any loss of forecasting accuracy. These findings suggest that the over-parameterization typically associated with regularization methods is not a necessary price for predictive accuracy in electricity price forecasting.

==> considered_methods.tex <==
% \section{Considered variable selection methods}\label{sec: variable selection methods}
\subsection{The considered variable selection problem}
In this study, we consider the multivariate modeling framework, where the 24-dimensional price series is modeled by a set of 24 univariate models \citep{zielweron2018}. Let $x^{(\ell)}_{d,h}, x^{(r)}_{d,h}$ be the load DA forecast and renewable DA forecast, for day $d$ hour $h$, and $x^{(gas)}_{d}, x^{(coal)}_{d}, x^{(oil)}_{d},x^{(eua)}_{d}$ be the TTF Gas, API2, Brent Oil and EUA Dec closing prices on day $d$, respectively. Moreover, let $z_{d} = (z_{d,1}, z_{d,2}, \ldots, z_{d,6})$ be a day-of-week dummy variable encoding the weekdays Tuesday through Sunday, by setting all its elements to zero except the element that identifies the day of the week, e.g. $(1, 0, 0, 0, 0, 0)$ represents Tuesday, $(0, 1, 0, 0, 0, 0)$ represents Wednesday. Inspired by the Lasso Estimated AutoRegressive (LEAR) model of \citet{Uniejewski2016} and \citet{lago2021}, we consider the following variable selection problem for each hour $h=1,\ldots,24$
\begin{equation}\label{eq: our variable selection problem}
    \begin{aligned}
        y_{d,h} = &\beta_{d,h,0} + \sum_{j=1}^7\sum_{i=1}^{24}\beta_{d,h,24(j-1) + i}y_{d-j,h-i} + \sum_{j=0}^7\sum_{i=1}^{24}\beta_{d,h,168 + 24j+i}x^{(\ell)}_{d-j,i} \\
        &+\sum_{j=0}^7\sum_{i=1}^{24}\beta_{d,h,360 + 24j+i}x^{(r)}_{d-j,i} + \sum_{i=1}^6 \beta_{d,h,552+i}z_{d,i} \\ &+ \beta_{d,h,559}x^{(gas)}_{d-2} + \beta_{d,h,560}x^{(coal)}_{d-2} + \beta_{d,h,561}x^{(oil)}_{d-2}+ \beta_{d,h,562}x^{(eua)}_{d-2} + u_{d,h},
    \end{aligned}
\end{equation}
meaning that we are considering a candidate set of $n = 562$ variables. We do not consider a yearly seasonal component explicitly in \eqref{eq: our variable selection problem} due to the pronounced yearly seasonality present in the load DA forecast variable.

Based on the general variable selection problem Section \ref{sec: variable selection problem} we describe in this section the considered variable selection methods. We refer to the references for each method for an in-dept description of each method.

\subsection{LASSO} % put references on its use in EPF
The Least Absolute Shrinkage and Selection Operator (LASSO) introduced in \citet{lasso} uses an $\ell_1$ penalty factor to introduce shrinkage and variable selection. First introduced in the context of EPF in \citet{Uniejewski2016}, they conclude that LASSO outperforms other variable selection methods, such as stepwise regression. Other uses of the LASSO in EPF include \citet{zielweron2018, lago2021} for day-ahead spot prices, and \citet{UNIEJEWSKI2019} for intraday prices. In the setting of Section \ref{sec: variable selection problem} the minimization problem solved in LASSO is the following
\begin{equation}\label{eq: lasso}
    \hat\beta = \underset{\beta \in \R^{n+1}}{\arg \min} \left\{ \left( y_t - \beta_0 - \sum_{i=1}^n \beta_i x_{ti} \right)^2 + \lambda \sum_{i=1}^n \abs{\beta_i} \right\},
\end{equation}
where $\lambda \geq 0$ is a tuning parameter to be decided by the user. Following \citet{lago2021}, we use the least angle regression (LARS) LASSO of \citet{efron} to select $\lambda$ according to the Akaike Information Criterion (AIC). 

\subsection{Elastic Net} % put references on its use in EPF
Introducing both an $\ell_1$ and an $\ell_2$ penalty, elastic net selects variables like LASSO and shrinks together the coefficients of correlated variables like ridge regression. While not as widely used as LASSO, elastic net was first used by \citet{Uniejewski2016} in the context of EPF, where it outperformed all considered variable selection methods, including LASSO, in terms of forecast accuracy. Other uses include \citet{MUNIAIN2020} for forecasting day-ahead prices in Germany, and \citet{AGRAWAL2019} for real-time predictions in the New England electricity market. The minimization problem to be solved in elastic net takes the form:
\begin{equation}\label{eq: elastic net}
    \hat\beta = \underset{\beta \in \R^{n+1}}{\arg \min} \left\{ \left( y_t - \beta_0 - \sum_{i=1}^n \beta_i x_{ti} \right)^2 + \lambda \left( \frac{1-\alpha}{2}\sum_{i=1}^n \abs{\beta_i} + \alpha\sum_{i=1}^n \beta_i^2 \right)\right\}, 
\end{equation}
where $\alpha \in [0,1]$ and $\lambda\geq0$ are tuning parameters. For $\alpha = 1$, elastic net reduces to the LASSO, while for $\alpha=0$ it becomes ridge regression. The shrinkage of correlated regressors is an especially useful feature in the context of EPF, where variables can be highly correlated. A disadvantage of elastic net, however, is the fact that it has two tuning parameters $\alpha, \lambda$ compared to just one in LASSO. An approach for determining $\alpha$ and $\lambda$ is to do a double grid search and use an information criterion to determine the optimal values. Following \citet{Uniejewski2016} we do a double grid search over exponentially decreasing $\lambda$'s and three values of $\alpha = 0.25, \alpha = 0.50, \alpha = 0.75$, and choose the pair $\{\lambda, \alpha\}$ based on the AIC. More specifically, for each $\alpha$ we construct the grid of $\lambda$'s as follows: define
$$
\lambda_{max} = \frac{\max_{j \in\{1, \ldots, n\}} |x_j^\top y|}{T\alpha},
$$
and set $\lambda_{min} = 10^{-3}\lambda_{max}$, then the grid is constructed as
$$
\lambda_m = \lambda_{max}\left( \frac{\lambda_{min}}{\lambda_{max}} \right)^{m/(M-1)}, \quad m = 0, 1, \ldots, M - 1.
$$

\subsection{Factor-Adjusted Regularized Model Selection (FarmSelect)}
Factor-Adjusted Regularized Model Selection (FarmSelect), proposed by \citet{FarmSelect}, is designed for high-dimensional regression problems in which the candidate covariates exhibit strong dependence. FarmSelect addresses this issue by decomposing the candidate variables into a small number of common factors and weakly correlated idiosyncratic components. Variable selection is then performed on the idiosyncratic components, while the estimated common factors are included as unpenalised regressors.

By removing the dependence attributable to a small number of common factors before applying regularisation, FarmSelect transforms the problem from one with highly correlated covariates to one with weakly correlated ones. The numerical results of \citet{FarmSelect} indicate that the method is superior to both LASSO and elastic net in terms of recovering the correct model specification in settings of highly correlated covariates.

Let $X =(x_1,\ldots,x_T)^\top \in \mathbb{R}^{T\times n}$ denote the observation matrix of the $n$ candidate covariates. FarmSelect assumes that the vector of candidate variables follows an approximate factor model of the form
$$
x_t = Bf_t + u_t, \qquad t=1,2,\ldots,T,
$$
where $x_t=(x_{t1},\ldots,x_{tn})^\top$, $f_t\in\mathbb{R}^\zeta$ is a vector of $\zeta \in \N$ latent common factors, $B\in\mathbb{R}^{n\times \zeta}$ is a factor loading matrix, and $u_t\in\mathbb{R}^n$ are the idiosyncratic components. In matrix form, the decomposition is
\begin{equation}\label{eq: factor model}
    X = FB^\top + U,
\end{equation}
where $F=(f_1,\ldots,f_T)^\top\in\mathbb{R}^{T\times \zeta}$ and $U=(u_1,\ldots,u_T)^\top\in\mathbb{R}^{T\times n}$.

\paragraph{Step 1: Estimation of approximate factor model}
Since the factors and loadings are unobserved, they are estimated by principal component analysis (PCA). Thus, for a given number of factors $\zeta$, the columns of $\hat F/\sqrt{T} = Q$ are the eigenvectors associated with the $\zeta$ largest eigenvalues of $XX^\top$. By the OLS estimator of $B$ we get
\begin{align*}
    \hat B &= X^\top \hat F(\hat F^\top \hat F)^{-1} \\
    & = X^\top \hat F (TQ^\top Q)^{-1} \\
    &= \frac{1}{T}X^\top \hat F
\end{align*}
from which the estimated idiosyncratic components follow as $\hat U = X-\hat F\hat B^\top$.

To specify the number of factors $\zeta$, \citet{FarmSelect} uses a modified eigenvalue-ratio criterion to select the minimum number such that the idiosyncratic components are weakly correlated. Specifically, $\hat \zeta$ is chosen according to
$$
\hat \zeta = \underset{0\leq \zeta\leq \zeta_{\max}}{\arg\min} \frac{\lambda_{\zeta+1}(XX^\top)+C_T}{\lambda_\zeta(XX^\top)+C_T},
$$
where $\lambda_\zeta(XX^\top)$ denotes the $\zeta$th largest eigenvalue of $XX^\top$, $\zeta_{\max} \in \N$ is a prescribed upper bound, and $C_T\in\R$. In the empirical application, we follow the implementation in the FarmSelect R package and choose $C_T=0$ while limiting ourselves to a maximum of 20 factors, $\zeta_{max}=20$.

\paragraph{Step 2: Factor-adjusted penalised regression}
FarmSelect replaces the original, strongly correlated regressors in $X$ with the estimated factors, $\hat F$, and idiosyncratic components, $\hat U$. While FarmSelect is applicable to generalized linear models and a broad class of penalised regression problems, we restrict attention to linear regression with an $\ell_1$ penalty (LASSO), as this is the setting we will be considering in the empirical application. In this case, the regression model reads:
$$
y_t = \beta_0\mathbf{1}_T+\hat F\gamma+\hat U\beta+\varepsilon_t,
$$
where $\gamma \in \R^{\hat\zeta}$ and $\beta\in \R^{n}$. Thus, by lifting the covariate space from $\R^n$ to $\R^{n+\hat\zeta}$, we replace the highly correlated variables in $X$ with weakly correlated ones. In the estimation, $\gamma$ are treated as nuisance parameter and are not penalised, whereas the coefficients $\beta$ associated with the idiosyncratic components are subject to regularisation. Hence, when using an $\ell_1$ penalty the FarmSelect estimator is
$$
(\hat \beta_0,\hat\gamma,\hat\beta) = \underset{\substack{ \beta_0\in\mathbb{R},\, \gamma\in\mathbb{R}^{\hat \zeta},\, \beta\in\mathbb{R}^n}}{\arg\min} \left\{\left( y_t -\beta_0 - \sum_{i=1}^{\hat\zeta} \gamma_i \hat f_{ti}- \sum_{i=1}^n \beta_i \hat u_{ti} \right)^2 + \lambda \sum_{i=1}^n |\beta_i| \right\},
$$
for $\lambda>0$. Equivalently, by solving the least squares problem with respect to $\gamma$ we get the profiled least squares problem
\begin{equation}\label{eq: profiled least squares}
    \hat\beta=\arg\min_{\beta\in\mathbb{R}^{n+1}}\left\{\frac{1}{2T} \left\| \hat M_Zy-\hat M_Z\hat U\beta\right\|_2^2+\lambda\|\beta\|_1 \right\},
\end{equation}
where $\hat M = I_T - \hat P$ and $\hat P = \hat F(\hat F^\top\hat F)^{-1}\hat F^\top$ are the projection matrices onto, and orthogonal to, the space spanned by the estimated factors. Thus, FarmSelect can be interpreted as removing the factor variation from the response variable and the idiosyncratic components and then applying LASSO to this factor-adjusted regression problem.

As for LASSO, we use the LARS LASSO to select $\lambda$ in FarmSelect based on the AIC. 

\subsection{One Covariate at a Time Multiple Testing}
The One Covariate at a Time Multiple Testing (OCMT) procedure proposed by \citet{OCMT} takes a fundamentally different approach to variable selection. Rather than inducing sparsity through coefficient penalisation, OCMT formulates variable selection as an iterative multiple-testing problem. At each stage, candidate covariates are tested individually using multiplicity-adjusted critical values, conditional on the variables selected in previous stages. Once no additional variables are selected, the final model is estimated by OLS. 

To the best of our knowledge, the OCMT procedure is yet to be applied in the context of EPF, but \citet{OCMT} draws some promising conclusions from their simulation study, motivating its inclusion. Although they conclude that no method dominates uniformly, they find that OCMT can yield lower false-selection rates and competitive or lower forecast errors than LASSO. Moreover, its low computational cost is attractive in a forecasting setting in which variable selection must be repeated across forecast origins and delivery periods. We outline the procedure below using the setting and notation introduced in Section \ref{sec: variable selection problem}.
\paragraph{Stage 1} In the first stage, we consider $n$ bivariate regressions\footnote{We emphasize the fact that in the OCMT one may condition in the first stage on a set of known covariates. That is, instead of considering bivariate regressions, one may consider regressions of $y_t$ on a vector $z_t$ of known pre-selected variables, an intercept, and, one at a time, $x_{ti}$ for $i = 1, 2,\ldots, n$: $$
y_t = z_t^\top a +  c_{i,(1)} + \phi_{i,(1)}x_{ti} + e_{ti,(1)}, \text{ for } t = 1, 2, \ldots, T.
$$
The procedure remains unchanged whether conditioning on a set of pre-selected variables or not.} of $y_t$ on an intercept and, one at a time, $x_{ti}$ for $i = 1, 2,\ldots, n$
$$
y_t = c_{i,(1)} + \phi_{i,(1)}x_{ti} + e_{ti,(1)}, \text{ for } t = 1, 2, \ldots, T,
$$
and denote the $t$-statistic of $\phi_{i,(1)}$ by $t_{\hat\phi_{T,i,(1)}}$ where $\hat\phi_{T,i,(1)}$ denotes the OLS estimator of $\phi_{i,(1)}$. We further denote by $\mathbbm{1}(A)$ the indicator function taking the value $1$ if $A$ is true, and $0$ otherwise. The first stage multiple testing estimator of $\mathbbm{1}(\beta_i \neq 0)$ is given by
$$
\widehat{\mathbbm{1}_{(1)}(\beta_i \neq 0)} = \mathbbm{1}\left( |{t_{\hat\phi_{T,i,(1)}}|} > c_p(n,\delta_1)\right), \text{ for } i=1,2,\ldots,n,
$$
where $c_p(n,\delta_1)$ is a critical value function defined as
\begin{equation}\label{eq: critical value function}
    c_p(n,\delta_1) = \Phi^{-1}\left( 1 - \frac{p}{2f(n,\delta_1)} \right),
\end{equation}
where $\Phi^{-1}$ is the inverse of the standard normal distribution function, $f(n,\delta) = cn^{\delta_1}$ for $c,\delta_1>0$, and $0<p<1$ is the significance level of the individual tests. The variables in the candidate set for which $\widehat{\mathbbm{1}_{(1)}(\beta_i \neq 0)} = 1$ are selected as signals or pseudo-signals. We denote by $k_{(1)}^s$ the number of selected variables in the first stage, the index set of the selected variables by $\mathcal{I}^s_{(1)}$, and the observation matrix of the selected variables by $X_{(1)}^s \in \R^{T \times k_{(1)}^s}$. Moreover, let $k_{(1)} = k_{(1)}^s$ be the total number of selected variables after stage 1, $X_{(1)} = (\mathbf{1}_T, X_{(1)}^s) = (x_{(1),1}, x_{(1),2}, \ldots, x_{(1),T})^\top  \in \R^{T \times k_{(1)}}$, $\mathcal{I}_{(1)} = \mathcal{I}_{(1)}^s$, and $\mathcal{N}_{(1)} = \{1,2,\ldots,n\} \setminus \mathcal{I}_{(1)}$. 

\paragraph{Stage $j>1$} In stage $j = 2,3,\ldots$ we consider $n- k_{(j-1)}$ regressions of $y_t$ on $x_{i,t}$ one at a time, for $i \in \mathcal{N}_{(j-1)}$, conditional on the variables in $X_{(j-1)}$:
$$
y_t = x_{(j-1),t}^\top \beta_{(j)} + \phi_{i,(j)}x_{ti} + e_{ti,(j)}, \text{ for } t=1, 2, \ldots, T.
$$
Denote by $t_{\hat\phi_{T,i,(j)}}$ the $t$-statistic of  $\phi_{i,(j)}$ where $\hat\phi_{T, i,(j)}$ denotes the OLS estimator of $\phi_{i,(j)}$, then variables for which $\widehat{\mathbbm{1}_{(j)}(\beta_i \neq 0)} = \mathbbm{1}\left( |t_{\hat\phi_{T,i,(j)}}| > c_p(n,\delta_2)\right) = 1$ are added to the set of already selected variables from stage $j-1$. As in the first stage, we denote by $k_{(j)}^s$ the number of selected variables in stage $j$, the index set of the selected variables by $S^s_{(j)}$, and the observation matrix of the selected variables by $X_{(j)}^s \in \R^{T \times k_{(j)}^s}$. We then update the total number of selected variables, the observation matrix of selected variables, the index set of selected variables, and the index set of variables not yet selected according to
\begin{alignat*}{2}
            X_{(j)} &= (X_{(j-1)}, X_{(j)}^s), \qquad\hat k_{(j)} &&=  k_{(j-1)} + k_{(j)}^s\\
            S_{(j)} &= S_{(j-1)} \cup S_{(j)}^s, \qquad\mathcal{N}_{(j)} &&= \{1,\ldots,n\} \setminus S_{(j)}.
\end{alignat*}
If $k_{(j)}^s >0$ we move onto stage $j+1$, whereas if $k_{(j)}^s = 0$, i.e. no variables are selected in stage $j$, the procedure terminates and the total number of selected variables is set to $k_{(j-1)}$. In case we terminate the procedure, the last step consists of an OLS regression of $y$ on the selected variables in $X_{(j-1)}$.

\subsection{Generalized OCMT (GOCMT)} %https://www.tandfonline.com/doi/full/10.1080/07474938.2024.2446864
A different procedure utilizing the factor model representation in \eqref{eq: factor model} to reduce correlation among covariates is the generalized OCMT (GOCMT) proposed by \citet{gocmt}. The proposed method builds upon the OCMT by conditioning on a set of pre-selected factors in every stage, thereby accounting for the common correlation across the covariates. Specifically, in the first stage, we consider $n$ regressions of the form
$$
y_t = c_{i,(1)} + \hat f_t^\top \gamma_{i,(0)} + \phi_{i,(1)}x_{ti} + e_{ti,(1)}, \text{ for } t = 1, 2, \ldots, T,
$$
and the variables are selected according to the same multiple testing estimator as in OCMT. 

Similarly, for subsequent stages $j=2,3,\ldots$ we condition on the factors and the variables selected in previous stages: for $i\in\mathcal{N}_{(j-1)}$ estimate
$$
y_t= \hat f_t^\top\gamma_{i,(j)}+x_{(j-1),t}^\top\beta_{i,(j)}+\phi_{i,(j)}x_{ti}+e_{ti,(j)}, \text{ for } t = 1, 2, \ldots, T.
$$
Selection, updating, and termination then proceed as in the standard OCMT procedure.

Again, PCA is used to estimate the factors, and, as in FarmSelect, we use the modified eigenvalue-ratio criterion with $C_T=0$ and $\zeta_{max}=20$ to select the number of factors.

\subsection{Boosting with Multiple Testing (BMT)}
Boosting with Multiple Testing (BMT), proposed by \citet{BMT}, builds on OCMT by combining its multiple-testing framework with forward stepwise variable selection. Whereas OCMT selects all candidate variables that pass the multiple-testing filter, BMT selects only the covariate with the largest absolute $t$-statistic. The remaining candidate variables are then moved onto subsequent stages, where they are retested conditional on the set of selected variables. As in the OCMT, the procedure then continues until no covariates pass the multiple-testing filter.

The stepwise selection of BMT is intended to reduce the selection of proxy variables, i.e., covariates with $\beta_i=0$ that nevertheless appear predictive because they are correlated with true signals. Once a signal has entered the model, the conditional significance of its proxies may disappear, allowing BMT to approximate the true DGP better. This property is particularly relevant for electricity price forecasting, where variables like lagged prices, load and renewable forecasts, and fuel prices are often strongly correlated. Further support for this is provided by the simulation study conducted in \citet{BMT}, where the authors conclude that BMT has better performance in terms of variable selection than OCMT and penalised regression methods - especially in cases of high multicollinearity. In addition, the authors also provide theoretical evidence that the OLS estimator based on BMT-selected variables is asymptotically equivalent to the oracle estimator that would be obtained if the true DGP was known in advance. 

Since BMT relies on the same conditional regressions and multiple-testing critical values as OCMT, we only describe the modifications that distinguish the two procedures. 
% Let
% $$
% S_{(0)} = \varnothing, \qquad \mathcal{N}_{(0)} = \{1,\ldots,n\},\qquad X_{(0)} = \mathbf{1}_T,
% $$
% where $S_{(j)}$ and $\mathcal{N}_{(j)}$ denote, respectively, the sets of selected and remaining candidate variables after stage $j$.

\paragraph{Stage 1}
As in the first stage of OCMT, consider the \(n\) bivariate regressions\footnote{Again, in the BMT one may condition on known pre-selected variables.}: for $i=1,2,\ldots,n$
$$
y_t = c_{i,(1)} + \phi_{i,(1)}x_{ti} + e_{ti,(1)}, \qquad t=1,2,\ldots,T.
$$
However, rather than selecting all variables that pass the multiple testing filter, BMT selects only the variable with the largest absolute $t$-statistic among these. Let $\mathcal{N}_{(0)}=\{1,2,\ldots,n\}$ and define
$$
\mathcal{C}_{(0)} = \left\{i\in\mathcal{N}_{(0)} : |t_{\hat\phi_{T,i,(j)}}| > c_p\!\left(n,\delta_2\right) \right\},
$$
then BMT selects the variable in the first stage according to
$$
i_{(1)} = \arg\max_{i_{(1)}\in\mathcal{N}_{(0)}} |t_{\hat\phi_{T,i,(1)}}|.
$$
The selected and remaining index sets, along with the matrix of selected variables after the first stage, are then given as
$$
S_{(1)}=\{i_{(1)}\}, \qquad \mathcal{N}_{(1)} = \mathcal{N}_{(0)}\setminus\{i_{(1)}\}, \qquad X_{(1)} = \left(\mathbf{1}_T,x_{i_{(1)}}\right).
$$

\paragraph{Stage $j>1$}
At stage \(j=2,3,\ldots\), each remaining candidate variable is tested separately conditional on the variables already selected. Thus, for each
$i\in\mathcal{N}_{(j-1)}$, we estimate
$$
y_t = x_{(j-1),t}^{\top}\beta_{(j)} + \phi_{i,(j)}x_{ti} + e_{ti,(j)}, \qquad t=1,\ldots,T,
$$
and compute the corresponding $t$-statistic
$t_{\hat\phi_{T,i,(j)}}$. Let
$$
\mathcal{C}_{(j)} = \left\{i\in\mathcal{N}_{(j-1)} : |t_{\hat\phi_{T,i,(j)}}| > c_p\!\left(n_{(j-1)},\delta_2\right) \right\},
$$
where $n_{(j-1)}$ is the cardinality of $\mathcal{N}_{(j-1)}$, i.e. the number of candidate variables remaining at stage $j$.
If $\mathcal{C}_{(j)}=\varnothing$, the procedure terminates and the final model is estimated by OLS using the variables contained in $X_{(j-1)}$. Otherwise, BMT selects only the most significant variable among those that pass the multiple-testing filter:
$$
i_{(j)} = \arg\max_{i\in\mathcal{C}_{(j)}} |t_{\hat\phi_{T,i,(j)}}|.
$$
The selected and remaining index sets and the matrix of selected variables are then updated according to
$$
S_{(j)} = S_{(j-1)}\cup\{i_{(j)}\}, \qquad \mathcal{N}_{(j)} = \mathcal{N}_{(j-1)}\setminus\{i_{(j)}\}, \qquad X_{(j)} = \left(X_{(j-1)},x_{i_{(j)}}\right).
$$
The procedure subsequently moves to stage \(j+1\).





